A Survey on Routing in Anonymous Communication Protocols

The Internet has undergone dramatic changes in the past 15 years, and now forms a global communication platform that billions of users rely on for their daily activities. While this transformation has brought tremendous benefits to society, it has also created new threats to online privacy, ranging from profiling of users for monetizing personal information to nearly omnipotent governmental surveillance. As a result, public interest in systems for anonymous communication has drastically increased. Several such systems have been proposed in the literature, each of which offers anonymity guarantees in different scenarios and under different assumptions, reflecting the plurality of approaches for how messages can be anonymously routed to their destination. Understanding this space of competing approaches with their different guarantees and assumptions is vital for users to understand the consequences of different design options. In this work, we survey previous research on designing, developing, and deploying systems for anonymous communication. To this end, we provide a taxonomy for clustering all prevalently considered approaches (including Mixnets, DC-nets, onion routing, and DHT-based protocols) with respect to their unique routing characteristics, deployability, and performance. This, in particular, encompasses the topological structure of the underlying network; the routing information that has to be made available to the initiator of the conversation; the underlying communication model; and performance-related indicators such as latency and communication layer. Our taxonomy and comparative assessment provide important insights about the differences between the existing classes of anonymous communication protocols, and it also helps to clarify the relationship between the routing characteristics of these protocols, and their performance and scalability.

==> sections/attacks.tex <==
\subsection{Nomenclature of Attacks}
There is a huge variety of attacks that an attacker can use against an anonymity protocol to break or at least reduce anonymity of the users~\cite{Raymond:2000:Survey}. 
%employing a wide range of active and passive techniques.
%\cite{Raymond:2000}
We present the most relevant attacks that could be applied to AC protocols. We cluster the attacks in the following categories: 

\paragraph{Active vs. Passive} In general we recognize two types of attacks, whether an adversary is active or passive. A passive adversary is able to listen and record traffic on network links, as well as to correlate messages that are entering and leaving the anonymity network or some parts of it. An active adversary, on the other hand, is not only able to monitor the network but also to modify and manipulate the network traffic. 

\paragraph{External vs. Internal} When an adversary uses only the communication channel (either passively or actively) without being a part of the network to mount an attack, then it is considered as an external attack. In contrary, an internal attack is mounted by an adversary who has some kind of control within the network such as controlling a fraction of the network or participates as a client.

\paragraph{Global vs. Local} 
A threat model usually specify how much of the network an adversary can monitor or manipulate, therefore we define two type of attacks, global and local. A local adversary has a control over a particular node, a small set of nodes, or some of the communication links within the network. On the other hand, a global adversary or observer, is a very powerful adversary that controls every network link between the clients and the nodes. A global adversary can theoretically correlate every user request to the anonymity network, and the final access that goes out from the anonymity network.

\paragraph{Adaptive vs. Static} A static adversary chooses a static set of resources such as nodes and communication links and is not able to adapt to any potential changes once the protocol has started. An adaptive adversary is more powerful adversary who can adapt his set of resources during the protocol run.  

==> sections/classification.tex <==
\subsection{Classification of Protocols}
\label{sec:classification}

In this section, we will classify routing protocols.



==> sections/deployability.tex <==
\subsection{Deployability}

\begin{enumerate}


\end{enumerate}

==> sections/freenet.tex <==
%\subsection{DHT-based systems}
\label{sec:freenet}


\emph{Freenet} is designed as a peer-to-peer censorship-resistant system for sharing storage pace. Freenet offers strong decentralization in order to provide privacy and robustness against attacks. The key design feature of Freenet is based on storage replication and plausible deniability. %Freenet has been extended to be used for other application such as Freenet sites, email, and messaging system. In Freenet 
Files are stored multiple times at the nodes and are indexed by binary file keys and can be looked up by their corresponding key. Each node has a dynamic routing table including the node information with the stored keys~\cite{Clarke:2001:FN}. The original design uses a heuristic deterministic routing using potentially all Freenet participating nodes choosing mostly neighborhood nodes (currently called Opennet mode). Freenet uses a adaptive routing using distributed hash tables with keys that are location-independent. Three methods are used for key construction: keyword-signed, key signed-subspace key, and content-hash key (for more details see \cite{Clarke:2001:FN}).The routing table is updated during time to achieve better performance. The replication of files provides resilience against node failure and node overloads.

In the Opennet mode, a heuristic-based and deterministic routing, a distance-directed depth-first search with backtracking, is used \cite{Roos:2014:FN} \cite{Clarke:2010:FN}. When a file request arrives at a node, including a key and a value for hops-to-live, if the file is not stored locally, the node looks up the node with the nearest key in the routing table and forwards the file request to the corresponding node. The node receiving the request repeats the process until either the file is found or the hops-to-live is reached. If the requested file is found the node forwards the file to the node from which he has received the request, stores a copy of the file locally and updates his routing table in order to optimize routing for future requests. If the node that is contacted is not responding, the nodes sends the request to the node with the second nearest key and if that is also unsuccessful he contacts the third nearest and so on. If the file is not retrieved within the hops-to-live number of hops then  the search is aborted and the file requester is informed.  The nodes that are forwarding the requested file back to the file requester change randomly the sender address  providing reasonable deniability for the node that has stored the file~\cite{Clarke:2001:FN}.

The Opennet mode was vulnerable to various attacks and in addition Freenet participating nodes were not protected and an attacker could easily find out whether a router is a participating Freenet node. In the Darknet mode such shortcomings are solved. In 2010, Freenet has been extended by a membership-concealing Darknet mode where trusted connection are used for routing \cite{Clarke:2010:FN}. In the Darknet mode, the user chooses the nodes from his trusted nodes \cite{Clarke:2010:FN}. The routing table is consisting nodes derived from a fixed graph that is the social graph of the node. In the Darknet mode, different than the Opennet mode, the routing table is not optimized during time and cannot include nodes that are not derived from the social graph of the node. Since, the Darknet mode is based on the trusted network of a user the structure of the network is following Kleinberg's small world model \cite{Kleinberg:2000:SWM}.



The relaying nodes only know their predecessor and the successor in order provide privacy. 
In Freenet the data is encrypted using symmetric encryption. 
The encryption/decrytion key is transfered either with the address or in the header of the file request~\cite{Clarke:2001:FN}.










\begin{comment}
\begin{center}
\begin{table}
\caption{Routing features of Freenet}
\centering
\begin{tabular}{| l | l |}
\hline
\textbf{Routing feature} & \textbf{Description} \\ \hline
Source routing & yes for Darknet no for Opennet \\ \hline
Random node selection & deterministic for both modes  \\ \hline
Congestion control & ? \\ \hline
%Decentralization & yes \\ \hline
Overlay network & yes  \\ \hline
Broadcast & no    \\ \hline
Using trust & yes for Darknet mode  \\ \hline
Bidirectional connections & yes \\ \hline
Topology  & small-world topology (by Jon Kleinberg) \\ \hline
Transport layer protocol & supports UDP  \\ \hline
% all schemes are invulnerable to traffic analysis
\end{tabular}
\end{table}
\end{center}
\begin{center}
\begin{table}
\caption{Security properties of Freenet}
\centering
\begin{tabular}{| l | l |}
\hline
\textbf{Security Property} & \textbf{Description} \\ \hline
Secure channel & between sender and receiver \\ \hline
Communication overhead & ?\\ \hline
DoS & not strongly vulnerable to DoS \\ \hline
Integrity & yes \\ \hline
Sender anonymity &   \\ \hline
Receiver anonymity & no  \\ \hline
Storage keeper anonymity & yes (by providing deniability)\\ \hline
Accountability & no    \\ \hline
Traffic analysis & vulnerable \\ \hline
Forward secrecy & no \\ \hline
% all schemes are invulnerable to traffic analysis
\end{tabular}
\end{table}
\end{center}
\end{comment}


==> sections/introduction_.tex <==
\section{Introduction}
The electronic communication over the years has evolved from a primitive
mechanism of delivering electronic messages to a global widespread public network that connects billions of users and businesses. The widespread presence of this public network (\ie the Internet) developed into a global multimedia platform where the users carry out sensitive and private information. While this transformation has brought a huge benefit for the users and businesses, it also created new privacy threats. By design, the early realizations of the protocols for electronic communication did not provide any means for protection of the transfered data.


The idea of anonymous (untraceable) communication is originating from David Chaum~\cite{Chaum:1981:mixnets} back in 1981, as a means of hiding the participants in an electronic email system. Over the last three decades an extensive research has been conducted that led to the development of novel protocols for anonymous communication. 

%Over the last three decades an extensive research has been 


%\paragraph{Motivation}

For preserving privacy of users, confidentiality by employing encryption techniques could be a possible solution. However, encryption alone is not considered enough as there could be statistical attacks on the encrypted data \cite{Wang:2013:Tor-Fingerprinting, Dyer:2012:Traffic-Analysis, Gilad:2012:Traffic-Analysis, Gong:2010:Traffic-Analysis, Liberatore:2006:TA, Sun:2002:web-stat, Wang:2003:Correlation-Traffic, Wang:2002:Correlation}.

Anonymous communication systems are designed to preserve privacy of users by hiding communication patterns from eavesdroppers. Even the anonymous communication systems have been exposed to various traffic analysis and fingerprinting attacks \cite{Houmansadr:2013:ParrotisDead, Panchenko:2011:OR-Fingerprinting, Chakravarty:2010:TA-BW, Murdoch:2007:Traffic-Analysis, Overlier:2006:Tor-hs, Murdoch:2005:Traffic-Analysis}. 
In \cite{Juarez:2014:Fingerprinting}, Juarez \etal evaluate website fingerprinting attacks on anonymous communication systems.
Cai \etal \cite{Cai:2014:Fingerprinting-Defenses} compare different website fingerprinting attacks and discuss their defenses.

%Research questions that we are tackling:



\iffalse
Anonymous communication \cite{Edman:2009:Survey}

Anonymous communication \cite{Ren:2010:Survey}

Anonymous communication \cite{Danezis:2008:Survey}

MixNet \cite{Sampigethaya:2006:MixNet}

\fi




\paragraph{Research Contributions}
In this work we aim at analyzing anonymous routing techniques. Our cotributions are as follows.
\begin{itemize}
 
 \item Classify routing characteristics for anonymous routing
 
 \item Review protocols
 
 %\item Briefly review frameworks for measuring anonymity

 %\item Categorisation
 
 \item Comparison based on characteristics we extracted
 
\end{itemize}

%\paragraph{Organization}
%\todo[inline]{Revise at the end.}
%This paper is structured as follows. In Section~\ref{sec:characteristics}, we describe general characteristics of routing protocols. Section~\ref{sec:protocols} reviews state-of-the-art routing protocols. Thereafter, in Section~\ref{sec:comparison}, we provide a comparative analysis based on general characteristics. Finally, Section~\ref{sec:conclusion} concludes our discussion.

==> sections/introduction__.tex <==
\section{Introduction}
Over the years  electronic communications have evolved from a primitive
mechanism of delivering electronic messages to a global widespread public network that connects billions of users and businesses. 
The Internet is today a global multimedia platform where the users and businesses carry out sensitive and private information. 
While this transformation has brought a huge benefit for the users and businesses, it has also created new privacy threats. 
By design, the early protocol realizations for electronic communication did not provide any means for protecting the transferred data neither the privacy of the communicating parties. The rapid evolution of the Internet and its involvement in the business and everyday life, clearly, has led to many concerns about its security and privacy. 
These concerns, mainly from the early designs and realizations, have been addressed with efforts to provide technical protections as well as a corresponding {\color{red}workarounds/solutions} on the top of the (insecure) underlaying protocols as a method for overcoming security and privacy problems. While confidentiality of data can be achieved using encryption techniques, the data is still linkable and the privacy is exposed to the attackers. 

In order to overcome the privacy problem, back in 1981, David Chaum~\cite{Chaum:1981:mixnets} proposed his idea of anonymous (untraceable) communication, as a means of implementing an anonymous email service. 

%The idea of anonymous (untraceable) communication was first proposed by David Chaum~\cite{Chaum:1981:mixnets} back in 1981, as a means of implementing an anonymous email service. 
Over the last three decades considerable attention has been paid to this problem, and extensive research has been conducted that have led to the development of novel protocols for anonymous communication. However, the research has demonstrated that these protocols are  continually followed/chased by variety of security problems [{\color{red}missing citation(s)}] and their performance fall short of the expectations of the users.


%\paragraph{Motivation}
%Encryption techniques provide a solution to protect the confidentiality of data. However, encryption alone is not considered enough as there could be statistical attacks on the encrypted data \cite{Wang:2013:Tor-Fingerprinting, Dyer:2012:Traffic-Analysis, Gilad:2012:Traffic-Analysis, Gong:2010:Traffic-Analysis, Liberatore:2006:TA, Sun:2002:web-stat, Wang:2003:Correlation-Traffic, Wang:2002:Correlation}.

One of the main aspects of anonymous communication is how data is sent through the network, \ie the routing strategy. The routing decision influence highly to the security and performance characteristics of the protocol. 
%One of the main aspects of anonymous communication is the routing strategy. 
%The routing decisions influence highly whether a communication can be traceable or not. 
In recent years a great deal of routing strategies have been proposed for anonymous routing. 
In this work we investigate routing strategies that are deployed for anonymous routing by proposing first a classification of all aspects relevant to anonymous routing. 
We thereafter evaluate various AC protocols based on our classification and finally discuss how their differences influence anonymity and performance of AC networks.

%Anonymous communication (AC) systems are designed to preserve privacy of users by hiding communication patterns from eavesdroppers. %Fateme: I dont know whether we need to address the following attacks here....?
%Even the anonymous communication systems have been exposed to various traffic analysis and fingerprinting attacks \cite{Houmansadr:2013:ParrotisDead, Panchenko:2011:OR-Fingerprinting, Chakravarty:2010:TA-BW, Murdoch:2007:Traffic-Analysis, Overlier:2006:Tor-hs, Murdoch:2005:Traffic-Analysis}. 
%In \cite{Juarez:2014:Fingerprinting}, Juarez \etal evaluate website fingerprinting attacks on anonymous communication systems.
%Cai \etal \cite{Cai:2014:Fingerprinting-Defenses} compare different website fingerprinting attacks and discuss their defenses.

%Research questions that we are tackling:



%Thereafter, we review related work and cD(s!7~b_OLR<
%onclude ou paper with the lessons we have learned by conducting this survey.

%\paragraph{Related Surveys and Articles}
%{\color{red}This might go to the very end of the paper}.
The fame of anonymous communication networks such as Tor has drastically changed in the past few years. 
The awareness of the users about their privacy on the Internet is the main engine and motivator for the researchers and scientist to contribute with different approaches and designs towards the common ultimate goal, usable anonymity on the Internet.   
<<<<<<< .mine
That is the main reason why anonymous communication protocols have been studied thoroughly in the past few years. There are a number of survey articles on anonymous communication~\cite{Ren:2010:Survey, Edman:2009:Survey, Danezis:2008:Survey} that discuss the different class of protocols from the aspect of anonymity and security, and also surveys on individual class of anonymous protocols \cite{Sampigethaya:2006:MixNet, Conrad:2014:I2PTor, AlSabah:2015:Tor-Survey}. Moreover, in \cite{Raymond:2000:Survey}, Raymond reviews various aspects of anonymous communication protocols including traffic analysis, attacks and design issues.
=======
That is the main reason why anonymous communication protocols have been studied thoroughly in the past few years. 

\todo[inline]{The following paragraph should stay in Introduction because it provides a concise overview of existing surveys. It could be important for convincing why we came up with a new survey.}
There are a number of survey articles on anonymous communication~\cite{Ren:2010:Survey, Edman:2009:Survey, Danezis:2008:Survey} that discuss the different class of protocols from the aspect of anonymity and security, and also surveys on individual class of anonymous protocols \cite{Sampigethaya:2006:MixNet, Conrad:2014:I2PTor, AlSabah:2015:Tor-Survey}. In \cite{Raymond:2000:Survey}, Raymond reviews various aspects of anonymous communication protocols including traffic analysis, attacks and design issues.
Back \etal \cite{Back:2001:Tradeoff} discuss trade-off of systems requiring low-latency anonymous communication and focus on Freedom networks \cite{Shostack:1999:Freedom, Back:2001:Freedom21} and PipeNets \cite{Dai:1996:PipeNet}. 
>>>>>>> .r103333
Hevia and Micciancio \cite{Hevia:2008:Indistinguishability} characterize anonymous communication protocols based on computational indistinguishability.
In \cite{Serjantov:2004:Anonymity}, Serjantov addresses how to quantify anonymous systems (mainly for email and browsing applications), describes a taxonomy of Mixnets and provides a list of attacks on them \cite{Shmatikov:2006:Mix-Attacks}. 
Attacks on Mixnets are presented in detail in \cite{Desmedt:2000:Break-Mix, Mitomo:2000:Mix-Attack, Serjantov:2003:Attacks, Serjantov:2003:PassiveAttack, Berthold:2003:Intersection-Attack, Danezis:2003:Heartbeat, Wikstroem:2004:Five-Mix-Attacks, Levine:2004:Mix-Attack, Danezis:2005:Attacks, Danezis:2005:Time-Mix, Diaz:2005:DummyTraffic, Mathewson:2005:Traffic-Analysis, Zhu:2005:Mix-Correlation, Danezis:2007:Mix-Break, Danezis:2007:2-Stat, Troncoso:2008:Disclosure, Troncoso:2009:Bayesian}.
Acquisti \etal \cite{Acquisti:2003:Economics} discuss economics of anonymity systems. 
They focus on providing incentives to participants for actively participating as nodes.
Serjantov and Danezis \cite{Serjantov:2003:Metric} and D{\'{\i}}az \etal \cite{Diaz:2003:Measurement} introduce information theoretic approaches for measuring anonymity based on probabilities distribution \ie probabilities of users sending and receiving the messages.

%Unlike the current survey articles that study the anonymity and security characteristics of the AC systems, our work addresses the routing characteristics of the protocols and their relation to the performance and scalability. 
Unlike the current survey articles that study the anonymity and security characteristics of the AC systems, our work addresses the routing characteristics of the protocols and their relation to the performance and scalability. 
%A recent survey \cite{Fra} compares and discusses anonymous communication protocols from the anonymity and security aspect. 

\paragraph{Research Contributions}
In this work we aim at analyzing anonymous routing techniques, our contributions are as follows.
\begin{itemize}
	
	\item Classifying routing characteristics for anonymous routing
	
	\item Describing the routing characteristics of the existing AC protocols
	
	%\item Briefly review frameworks for measuring anonymity
	
	%\item Categorisation
	
	\item Comparing the AC protocols based on characteristics we extracted for our classification
	
	\item Discuss the relevance between routing decisions and their influence on anonymity and security
	
\end{itemize}


The remainder of this paper is organized as follows. 
In the Section~\ref{sec:characteristics}, we elaborate on our classification for anonymous routing and describe the routing features and dimension that we are considering for our evaluation. 
Moreover, we also describe the performance features that we consider for the evaluations. 
In Section \ref{sec:comparison}, we demonstrate the evaluations in two tables.
In Section \ref{sec:protocols}, we briefly describe the AC protocols that we have chosen for our survey.
Moreover in Section \ref{sec:discussion}, we discuss the relevance between routing decisions and security and anonymity goals.

%\paragraph{Organization}
%\todo[inline]{Revise at the end.}
%This paper is structured as follows. In Section~\ref{sec:characteristics}, we describe general characteristics of routing protocols. Section~\ref{sec:protocols} reviews state-of-the-art routing protocols. Thereafter, in Section~\ref{sec:comparison}, we provide a comparative analysis based on general characteristics. Finally, Section~\ref{sec:conclusion} concludes our discussion.

==> sections/others.tex <==
\subsection{Other Systems}
\label{sec:others}

\todo[inline]{Tor recent extension \cite{Weinberg:2012:StegoTorus}. This comment has to be moved to Tor section.}

\todo[inline]{Very recent related work on hidden services \cite{Biryukov:2013:HiddenServices}. This comment has to be moved to Tor section.}

\todo[inline]{Attacks on TOR \cite{Jansen:2014:Tor-Sniper, Barbera:2013:CellFlood}. This comment has to be moved to Tor section.}

\todo[inline]{DoS on TOR \cite{Danner:2012:DoS-Tor}. This comment has to be moved to Tor section.}

\todo[inline]{If possible, we can adjust the following systems with description of existing protocols. Otherwise, we can list all systems under this subsection.}

%Anonymizer \cite{Anonymizer:2015}.

%Proxies for anonymous routing \cite{Reed:1996:Proxies}.

Hordes \cite{Shields:2000:hordes, Levine:2002:Hordes}. (What is this?)

Freedom \cite{Shostack:1999:Freedom, Back:2001:Freedom21}.

%Salsa \cite{Nambiar:2006:Salsa}.
%
%GAP \cite{Bennett:2003:GAP}.

P5 \cite{Sherwood:2002:P5}.

==> sections/p2p.tex <==
\subsection{P2P}
\label{sec:p2p}



\paragraph{I2P}
I2P is a message-oriented, peer-to-peer-based low latency anonymous communication network. The network was mainly designed to enable fully anonymous communication between two parties inside the network\cite{timpanaro2012i2p}\cite{timpanaro2011monitoring}.

The routing protocol in I2P is called \emph{Garlic Routing}, it is a source-routed tier-based randomized routing \cite{schimmeri2p}. The description of I2P's routing is retrieved from \cite{garlic-routing}, \cite{tunnel-routing}, \cite{schimmeri2p}, and \cite{conradshirazi}.
There are two types of tunnels; client tunnels and exploratory tunnels. Client tunnels are used application traffic and exploratory tunnels are used to send administrative information. Peer selection differs for the two types of tunnels.
For client tunnels, node selection in I2P is randomized with a bias towards nodes which had previously high performance. 
The nodes are categorized into tiers (called peer profiling); the nodes previous performance (response times) and reliability (uptime) are used for this categorization. 
Three types of tiers are defined in I2P: high capacity, fast, and standard. Communication channels are called tunnels in I2P. 
For client tunnels peers are selected randomly from the nodes that are categorized as fast tier nodes. 
For exploratory tunnels, peers are selected randomly from the set of nodes that are categorized as standard tier. 
In I2P, anonymity (both sender and receiver anonymity) is given by the probabilistic node selection and the use of encryption. 

message
%Congestion control in I2P is provided by using packet switching.  

\begin{center}
\begin{table}
\caption{Routing features of I2P}
\centering
 \begin{tabular}{| l | l |}
  \hline
  \textbf{Routing feature} & \textbf{Description} \\ \hline
   Source routing & yes \\ \hline
   Random node selection & nondeterministic but not uniform  \\ \hline
   Congestion control & packet switching \\ \hline
   %Decentralization & yes \\ \hline
   Overlay network & yes  \\ \hline
   Broadcast & no    \\ \hline
   Using trust  & no \\ \hline
   Bidirectional  connections & no \\ \hline
   Topology & nodes/users are fully\\ \hline% \\connected   except nodes \\from the /16   IP subnet,\\ nodes often \\  have the rich club connectivity  \\ property \\ \hline
   Transport layer protocol & supports TCP and UDP  \\ \hline
   % all schemes are invulnerable to traffic analysis
   
 \end{tabular}

\end{table}
\end{center}

\begin{center}
\begin{table}
\caption{Security properties of I2P}
\centering
 \begin{tabular}{| l | l |}
  \hline
  \textbf{Security Property} & \textbf{Description} \\ \hline
   Secure channel & Between sender and receiver \\ \hline
   Communication overhead & ? \\ \hline
   DoS & vulnerable to DoS \\ \hline
   Integrity & guaranteed \\ \hline
   Sender anonymity & yes \\ \hline%(unless all three nodes \\  chosen for communication\\ path collude) \\ \hline
   Accountability & no\\ \hline    
   Traffic analysis & vulnerable \\ \hline
   Forward secrecy& yes\\ \hline
   %Deniability& yes\\ \hline
   % all schemes are invulnerable to traffic analysis
   
 \end{tabular}


\end{table}
\end{center}
%Unlinkability

%Resistance against traffic analysis attacks: since I2P is a low latency ACN, theoretically traffic analysis attacks (timing attacks) are possible.

%Forward secrecy: I2P has a non deterministic node selection, however the node selection is biased toward fast nodes. 

%Sender and/or receiver anonymity: both are provided by the non-deterministic routing strategy and the end to end encryption. As of February 2013 I2P has around 20 000 users (size of sender anonymity set). 

%Accountability: I2P provides no accountability options.

%Deniability: 

%Availability/resilience: There have been several DoS attack schemes introduced for I2P. 

%Unobservability:

\paragraph{Freenet}
Freenet is a peer-to-peer network that was designed as a censorship-resistant publication system where the Freenet users share their storage pace with each other \cite{DBLP:conf/pet/RoosSHS14}. Freenet has been extended to be used for other application such as Freenet sites, email, and messaging system. The original design uses a heuristic deterministic routing using potentially all Freenet participating nodes choosing mostly neighborhood nodes (currently called Opennet mode).  In 2010, Freenet has been extended by a membership-concealing Darknet mode where trusted connection are used for routing \cite{clarke2010darknet}. The Darknet mode is intended to prevent various attacks and improve the anonymity and security of Freenet.

%Routing protocol: the routing in Freenet differs for the two modes. For the Opennet mode has  a deterministic heuristic (?) routing strategy \cite{} is used and the Darknet mode uses a .... trusted connections \cite{clarke2010darknet}, \cite{}.%4,5,6 from google docs


In the Opennet mode for file storage and retrieval a heuristic deterministic routing, a distance-directed depth-first search, is used \cite{DBLP:conf/pet/RoosSHS14}. The sender address is probabilistically changed by one of the nodes on the way. Anonymity is provided by enabling deniability.

In the Darknet mode, nodes only connect to manually chosen trusted nodes \cite{clarke2010darknet}, \cite{}. %Roos et al. have analyzed the Darknet routing in \cite{}.% [17] google docs

\begin{center}
\begin{table}
\caption{Routing features of Freenet}
\centering
 \begin{tabular}{| l | l |}
  \hline
  \textbf{Routing feature} & \textbf{Description} \\ \hline
   Source routing & yes for Darknet no for Opennet \\ \hline
   Random node selection & deterministic for both modes  \\ \hline
   Congestion control & ? \\ \hline
   %Decentralization & yes \\ \hline
   Overlay network & yes  \\ \hline
   Broadcast & no    \\ \hline
   Using trust & yes for Darknet mode  \\ \hline
   Bidirectional connections & yes \\ \hline
   Topology  & small-world topology (by Jon Kleinberg) \\ \hline
   Transport layer protocol & supports UDP  \\ \hline
   % all schemes are invulnerable to traffic analysis
   
 \end{tabular}

\end{table}
\end{center}
\begin{center}
\begin{table}
\caption{Security properties of Freenet}
\centering
 \begin{tabular}{| l | l |}
  \hline
  \textbf{Security Property} & \textbf{Description} \\ \hline
   Secure channel & between sender and receiver \\ \hline
   Communication overhead & ?\\ \hline
   DoS & not strongly vulnerable to DoS \\ \hline
   Integrity & yes \\ \hline
   Sender anonymity &   \\ \hline
   Receiver anonymity & no  \\ \hline
   Storage keeper anonymity & yes (by providing deniability)\\ \hline
   Accountability & no    \\ \hline
   Traffic analysis & vulnerable \\ \hline
   Forward secrecy & no \\ \hline
   % all schemes are invulnerable to traffic analysis
   
 \end{tabular}
\end{table}
\end{center}


%\subsection{Gnunet}
%Gnunet is designed as a censorship resistant file sharing system. Recently it has expanded into other applications. Gnunet basically provides an anonymous DNS system. The key idea here is to use pseudonyms


==> sections/pairwise.tex <==
\subsection{Pairwise Comparison of Characteristics}
\label{sec:pairwise}

TODO


==> sections/relatedwork_.tex <==
\section{Related Work}
\todo[inline]{We have to cite here all existing surveys (on anonymous communication and individual protocols) and point out how we are different.}

\todo[inline]{Group the this subsection based on same categories.}

There are a number of survey articles on anonymous communication \cite{Ren:2010:Survey, Edman:2009:Survey, Danezis:2008:Survey} and individual anonymous protocols \cite{Sampigethaya:2006:MixNet, Conrad:2014:I2PTor, AlSabah:2015:Tor-Survey}. 

In \cite{Raymond:2000:Survey}, Raymond reviews various aspects of anonymous communication protocols including traffic analysis, attacks and design issues.

Hevia and Micciancio \cite{Hevia:2008:Indistinguishability} characterize anonymous communication protocols based on computational indistinguishability.

Back \etal \cite{Back:2001:Tradeoff} discuss trade-off of systems requiring low-latency anonymous communication and focus on Freedom networks [CITE] and PipeNets [CITE].

% There are a number of proposals for devising metrics for measuring anonymity.
Edman \etal \cite{Edman:2007:Combinatorial} devise an information-theoretic metric for quantifying anonymity.

In \cite{Serjantov:2004:Anonymity}, Serjantov addresses how to quantify anonymous systems (mainly for email and browsing applications), describes a taxonomy of Mixnets and provides a list of attacks on them \cite{Shmatikov:2006:Mix-Attacks}. Attacks on Mixnets are presented in detail in \cite{Desmedt:2000:Break-Mix, Mitomo:2000:Mix-Attack, Serjantov:2003:Attacks, Serjantov:2003:PassiveAttack, Berthold:2003:Intersection-Attack, Danezis:2003:Heartbeat, Wikstroem:2004:Five-Mix-Attacks, Levine:2004:Mix-Attack, Danezis:2005:Attacks, Danezis:2005:Time-Mix, Diaz:2005:DummyTraffic, Mathewson:2005:Traffic-Analysis, Zhu:2005:Mix-Correlation, Danezis:2007:Mix-Break, Danezis:2007:2-Stat, Troncoso:2008:Disclosure, Troncoso:2009:Bayesian}.

Acquisti \etal \cite{Acquisti:2003:Economics} discuss economics of anonymity systems. They focus on providing incentives to participants for actively participating as nodes.

Serjantov and Danezis \cite{Serjantov:2003:Metric} and D{\'{\i}}az \etal \cite{Diaz:2003:Measurement} introduce information theoretic approaches for measuring anonymity based on probabilities distribution \ie probabilities of users sending and receiving the messages.

% D{\'{\i}}az \etal \cite{Diaz:2003:Measurement} propose an information theoretic model to quantify anonymity, considering attackers that have access to the probability distribution.

Backes \etal \cite{Backes:2013:AnoA} formalise the concept and propose a framework for analysing anonymous communication protocols. In \cite{Backes:2014:MATor}, they extend the framework to monitor the anonymity of the Tor [CITE] path selection. In \cite{Backes:2014:TUC}, they propose a framework for proving anonymity guarantees in the presence of time-sensitive adversaries, \ie a framework capable of modelling the traffic-related timing attacks against Tor.

In \cite{Shmatikov:2004:Analysis}, Shmatikov employs a probabilistic model checking approach to analyze the Crowds system for anonymous Web browsing.

In \cite{Wright:2002:Degradation}, Wright \etal investigate attacks that degrade anonymity of the protocols.

In \cite{Camenisch:2005:Formal-Onion}, Camenisch and Lysyanskaya provide a formal definition of onion routing in the universally composable framework.

Pfitzmann and Waidner \cite{Pfitzmann:1986:Unobservability} discuss design options of establishing communication networks without observing communicating parties.

==> sections/security.tex <==
\subsection{Security ?Requirements?} 
Protocols for anonymous communication need to provide a set of certain security guarantees. We identify the following list of security properties.

\begin{enumerate}
%	\item{\textbf{Attacker Model}}

	\item{\textbf{Anonymity.}} Anonymity is the state of being not identifiable within a set of subjects, \emph{the anonymity
set}. The anonymity set is defined as a set of all possible subjects~\cite{Pfitzmann:2010:ATerminology}, and may vary over time. With respect to the user's role in a communication system, Pfitzmann and Hansen~\cite{Pfitzmann:2010:ATerminology} define sender and recipient anonymity.
	\begin{itemize}
	\item \textbf{Sender anonymity.} A sender of a message may be anonymous only within a set of potential senders \ie \emph{sender anonymity set}. The sender anonymity set might be a subset of all users who might send a message. 
	
%	The sender of a messages is untraceable. TODO: revise.
 
	\item \textbf{Recipient anonymity.} A recipient of a message may be anonymous only within a set of potential recipients. 
	
%The recipient of a messages is untraceable. TODO: revise.
 

	\end{itemize}
		\item{\textbf{Unlinkability.}} This property ensures that a user may make arbitrary number of sessions or request without any other party to be able to associate these requests together. {\color{red}Fateme: I think we should extend the definition of unlinkability of two subjects}

	\item{\textbf{Forward secrecy.}} Forward secrecy is considered as a quite important security property for protocols for anonymous communication.
This property guarantees that \textbf{after} a protocol session is expired, if an adversary gets access to all parties in the protocol and learn their secret information such as secret keys, the security properties still hold.
We grant \textit{eventual} or \textit{immediate} forward secrecy depends of the expiration of the key. 
When all past sessions remain secret immediately after their expiration even if the private key is disclosed, we call this property immediate forward secrecy. Otherwise it is called eventual forward secrecy.
{\color{red} Forward secrecy/anonymity: Once a session ends and the session identifiers
used to associate nodes in the circuit, and symmetric keys used to protect
the node identities and message contents, are irrecoverable even if all OR
nodes in the circuit are subsequently compromised.}
	\item{\textbf{Integrity.}} The protocol implements a mechanism for integrity checking. If the protocol detects message tempering, it drops the message or applies a certain policy.
	%\item{\textbf{No trusted third party.} The protocol does not require a single trusted third party. We also grant this property to protocols that relay on a third party such as directory server which can be distributed.}

	%\item{\textbf{Resilient to a global observer.}} The protocol solves the problem with global observer, which in theory can follow end-to-end traffic. {\color{red}I think this doesn't make sense...better we add here global passive observer.}

%	\item{\textbf{Availability}}	\begin{itemize}
\item{\textbf{\color{red}Censorship resistance.}} The protocol implements a special mechanism in order to bypass internet censorship. We also grant this property if the protocol includes mechanism that help to bypass filtering and in particular possible blocking of the anonymity protocol. 
%\end{itemize}
\item{\textbf{Accountability.}} The protocol implements certain kind of accountability mechanism. The mechanism could be in a form of traceability, or non-repudiation (or deniability)~\cite{diaz:2007:accountable }.
%	\begin{itemize}
%\item Non-repudiation
%\item Traceability

%\end{itemize}

	
%	\item{\textbf{Prevent traffic analysis.}}

	
\end{enumerate}
Security properties that an ACN offers are influenced by non-technical and technical factors. For example, a bigger anonymity set increases the degree of anonymity that a system is offering because a larger set increases the uncertainty of the identity of the sender. The size of the anonymity set depends on the number of users that relay their communication through the ACN. Hence, a higher number of users for an ACN provides better sender anonymity. 
Routing features described in Section \ref{routing} also influence the degree of anonymity that a network offers. 
For example node selection method highly influences anonymity. In particular, non-deterministic node selection is often the common technique to provide anonymity in ACNs; in particular uniform node selection is supporting anonymity highly, because it makes it hard to guess the identity of the sender from between the anonymity set. Uniform random node selection helps the network to resist against deanonymizing attempts by an adversary, by making it harder to predict which nodes are selected for the same channel [path?relay sequence?] and hence making node coercions that leads to successful deanonymization expensive for the adversary. However, due to performance considerations, routing policies often do not select each possible route with the same probability; preference is given to high-performance nodes. Therefore, often node selection is a trade-off between high anonymity and optimizing performance. 
{\color{red}Note that for low-latency ACNs, the communication is assumed to be anonymous as long as an attacker is unable to gain control over first and last node relaying the communication at the same time (eliminating the threat of correlation, e.g. by timing,  attacks)}. Hence, selecting nodes from different /16 subnet IP address families makes it harder to control a path by nodes that have been set up by the adversary. %the ISP administrator or an autonomous system administrator. 
Furthermore, encrypting the communication content and the meta data supports anonymity by disguising the information about the sender and receiver of a message. However, encryption often does not hide the fact that the node is participating in the anonymous communication network but rather hides the role that the subject is having, e.g., being the sender of a communication, a relaying node, or the receiver of the communication.  

Two sessions or requests might be linked to each other by the meta data that they leave such as IP address, hence disguising the IP address supports unlinkability. Two subjects might be linked to each other by (tracing) their common communication path, hence non-deterministic node selection makes it hard for the adversary to guess before hand, which relays to coerce for tracing the communications successfully. Moreover, selecting nodes from different  subnet families supports unlinkability of two subjects because the it makes it harder for the adversary to set up nodes which happen to (all, or both) in the communication path of the the two users.

TODO Milivoj Forward security. 

TODO Integrity (Fateme: I am nor sure if we need to say much here since it would be not too relevant to the topic of our survey). 

TODO Censorship resistance (For example, the bridges in Tor).

TODO Milivoj Accountability. 

==> sections/table.tex <==
	
\begin{flushleft}

\begin{landscape}

\begin{table}[t!]


\begin{tabu}{ lll |[1pt] l | l | l | l | l | l | l |[1.5pt] l | l | l | l | l | l | l |[1.5pt] l | l | l | [1.5pt] l | l | l | [1.5pt] }


\tabucline[1pt]{4-23}


& &
& \multicolumn{7}{c|[1.5pt]}{\thead{\textbf{Routing}}}
& \multicolumn{7}{c|[1.5pt]}{\thead{\textbf{Security}}}
& \multicolumn{3}{c|[1.5pt]}{\thead{\textbf{Performance}}}
& \multicolumn{3}{c|[1.5pt]}{\thead{\textbf{Deployability}}}

\\ \tabucline[1pt]{4-23}

& &
& \makecell[c]{\begin{turn}{90} \makecell[c]{\scriptsize Routing \\ Type} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{\scriptsize Node \\ Selection} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{\scriptsize Connection\\Type} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Topology} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{P2P} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Network \\ View} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Directory \\ Service} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Anonymity} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Forward \\ Secrecy} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{{\color{red}Path Length} \\ {\color{red}Nodes Contacted}} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Unlinkability} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Accountability} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Integrity} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Confidentiality} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Latency} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Congestion \\ Control} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Communication \\ Complexity} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Implemented} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Scalability} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{TCP/IP Layer} \end{turn}}

\\ \hline


\multicolumn{1}{|c|}{\multirow{5}{*}{\thead{\emph{\textbf{Mixnet-based}} \\ \emph{\textbf{protocols}}}}}

& \multicolumn{1}{l|}{Chaum's MixNet}
& \cite{Chaum:1981:mixnets}
& \source & \deterministic  & \bi & \fullyc,\partiallyc & \no & \full & \yes & \both & \no & & \no & \no & ? & ? & \high & \no & & \no & & -

\\ \cline{2-23} 

\multicolumn{1}{|c|}{}
& \multicolumn{1}{l|}{Cypherpunk}
& \cite{Parekh:1996}
& \source & \nondetuni & \bi & \fullyc & \no &\full & \yes & \sender & & & \yes & \no & & \no & \high & \no & & \yes & \yes & 

\\ \cline{2-23} 

\multicolumn{1}{|c|}{}
& \multicolumn{1}{l|}{Mixmaster}
& \cite{moller:2003:mixmaster}
& \source & \nondetuni & \uni &\fullyc & \no  & \full & \yes & \sender & \yes & & \yes & \no & \yes & \no & H & \no & & \yes & ? & email 

\\ \cline{2-23}

\multicolumn{1}{|c|}{}
& \multicolumn{1}{l|}{Babel}
& \cite{Babel:1996}
& \source & \nondetuni & \bi & \fullyc & \no & \full & \yes & \both & & & \yes & \no &  & \no & H & \no & & \yes & & 

\\ \cline{2-23}

\multicolumn{1}{|c|}{}
& \multicolumn{1}{l|}{Mixminion}
& \cite{Danezis:2003:mixminion}
& \source & \nondetuni & \bi &\fullyc  & \no &\full & \yes &\both & \yes & & \yes & \no & \yes & \no & H & \no & \yes & \yes & \yes & 

%\\ \hline

\\ \cline{2-23}

\multicolumn{1}{|c|}{}
& \multicolumn{1}{l|}{Web Mixes}
& \cite{Berthold:2000:JAP}
& \source & \deterministic & \bi & \partiallyc & \no & \full & \yes & \sender & & & \yes & \no & \yes & \yes & L & \no & \yes & \yes & \yes & 

\\ \hline


% Anonymity \recipient \both 
% \boxtimes (fully) \Box (partial)
\multicolumn{1}{|c|}{\multirow{4}{*}{\thead{\emph{\textbf{DCNet-based}} \\ \emph{\textbf{protocols}}}}}
& \multicolumn{1}{l|}{{Chaum's DCNet}}
& \cite{Chaum:1988:DCNets}
& \source & \deterministic & \uni & \fullyc & \yes & \full & \yes & \both & \yes & $N$ & \yes & \no & \no & \no & \high & \no & \full & \no & \mini & Application

\\ \cline{2-23} 

\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Herbivore}
& \cite{Goel:2003:Herbivore}
& \source & \deterministic & \uni & \mostlyc & \yes & \partially & \yes & \both & \yes & $k$ & \yes & \no & \yes & \no & \high & \yes & \partially & \yes & \partially & IP

\\ \cline{2-23}

\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Dissent}
& \cite{Corrigan-Gibbs:2010:Dissent}
& \source & \deterministic & \uni & \fullyc & \yes & \full & \yes & \both & \yes & $N$ & \yes & \yes & \yes & \no & \high & \no & \full & \yes & \mini & Application

\\ \cline{2-23}

\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Verdict}
& \cite{Corrigan-Gibbs:2013}
& \source & \deterministic & \uni & \mostlyc & \yes & \partially & \yes & \both & \yes & $N$ & \yes & \yes & \yes ? & \no & \high & \no & \full & \yes & \mini & Application

\\ \hline


\multicolumn{1}{|c|}{\multirow{2}{*}{\thead{\emph{\textbf{Onion/Garlic}} \\ \emph{\textbf{routing}}}}}
& \multicolumn{1}{l|}{Tor}
& \cite{Dingledine:2004:Tor}
& \source & \nondetnonuni & \bi & \mostlyc & \no & \full  &\yes& \sender & \yes & 3 & \yes & \no & \no & \no & \low & \yes& & \yes& \yes&TCP

\\ \cline{2-23}

\multicolumn{1}{|l|}{\multirow{2}{*}{}}
& \multicolumn{1}{l|}{I2P}
& \cite{Web:2014:I2P}
& \source & \nondetnonuni & \uni & \mostlyc& \yes  & \full  & \yes& \sender & \yes & 3-4 & \yes & \no & \yes & \yes & \low &\yes & & \yes & \yes& TCP,UDP

%\\ \cline{2-23}

\\ \cline{2-23}

\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Pisces}
& \cite{Mittal:2013:Pisces}
& \source& \nondetuni&\bi &\partiallyc & \yes & \full & \no & \sender & \yes &3 & \yes & \no & \yes & \yes & \low & & & \no & \yes &TCP,UDP

\\ \hline
% producer & consumer
\multicolumn{1}{|c|}{\multirow{3}{*}{\thead{\emph{\textbf{DHT routing}}}}}
& \multicolumn{1}{l|}{Freenet/Darknet}
& \cite{Clarke:2010:FN}
& \source & \deterministic & \bi &\partiallyc  & \yes & \partially  & \no&\sender & \yes & $v$ & \yes & \no & \yes & \yes & -& & & \yes & \yes& Content sharing

\\ \cline{2-23}

\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Freenet/Opennet}
& \cite{Clarke:2001:FN}
& \hop & \deterministic & \bi &\partiallyc  & \yes &\partially  & \no&\sender &\no & $v$ & \yes & \no & \yes& \yes & -& & &\yes & \yes&Content sharing

\\ \cline{2-23}

%\\ \hline


%\iffalse
%initiator and responder anonymity
\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Gnunet}
& \cite{Bennett:2002:GN}
& \hop & \deterministic & \bi&\mostlyc &\yes &  \partially &\no &\both &  & $v$ &\yes &\no &\no &\no & -& & &\yes &\yes & Content sharing

\\ \hline

%\fi


\multicolumn{1}{|c|}{\multirow{2}{*}{\thead{\emph{\textbf{NG Internet}}}}}
& \multicolumn{1}{l|}{LAP}
& \cite{Hsiao:2011:LAP}
& \hop & \deterministic & \bi & & \no & \full & \no& \both & \no & & \yes & \no & \no& \no& \low &\yes & & \no & \yes &

\\\cline{2-23}

\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Dovetail}
& \cite{Sankey:2014:Dovetail}
& \hop &\deterministic &\bi & & \no &\full  & &\both & & & \yes& \no&\no & \no& \low & & & \no &\yes&

\\ \hline


\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Crowds}
& \cite{Reiter:1998:Crowds}
& \hop &\nondetnonuni & \bi & \fullyc&  \yes & \full & \yes & \sender &\yes & $v$ & \yes & \no & \no & \no &\low & & & \no &\yes & TCP (web browsing)

\\ \hline


\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Tarzan}
& \cite{Freedman:2002:Tarzan}
& \source& \nondetnonuni& \bi&  \mostlyc&\yes  & \partially &\no&\both  & & $v$ &\yes & \no &\yes  &\no &\low & & &\no & \yes & UDP

\\ \hline


\end{tabu}

\begin{minipage}{\linewidth}

\source Source routing \\
\hop Hop-by-hop routing \\

\yes Yes \\
\no No \\
\canbeboth Can be both \\

\deterministic Deterministic \\
\nondetuni Non-deterministic and uniform \\
\nondetnonuni Non-deterministic and non-uniform \\

\uni Uni-directional \\
\bi Bi-directional \\

\fullyc Fully-connected \\
\mostlyc Mostly-connected \\
\partiallyc Partially-connected \\
% \notc Not-connected ({\color{red} REMOVE: It will not happen}) \\

\sender Sender anonymity \\
\recipient Recipient anonymity ({\color{red} REMOVE: It will not happen}) \\
\both Both sender and recipient anonymity \\

$N$ Number of nodes in the network \\
$k$ Clique size, where number of cliques are $\lfloor N/k \rfloor$ \\
$v$ Variable, where $ 1 < v < N$ \\

\full Full \\
\partially Partial \\
\mini Minimal \\

\low Low \\
\high High \\

- Not applicable \\

\todo[inline]{\color{blue}{Move Nodes Contacted after Node Selection.}}

\end{minipage}

\end{table}

\end{landscape}

\end{flushleft}

==> sections/table_new.tex <==
	
\begin{flushleft}

\begin{landscape}

\begin{table}[t!]


\begin{tabu}{ lll |[1pt] l | l | l | l | l | l | [1.5pt] l | l | l | l |[1.5pt] l | l | l | [1.5pt] l | l | l | l | l | [1.5pt]  }


\tabucline[1pt]{4-21}


& & 
& \multicolumn{6}{c|[1.5pt]}{\thead{\textbf{Network Structure}}} 
& \multicolumn{4}{c|[1.5pt]}{\thead{\textbf{\makecell{Routing \\ Information}}}}
& \multicolumn{3}{c|[1.5pt]}{\thead{\textbf{\makecell{Communication \\ Model}}}}
& \multicolumn{5}{c|[1.5pt]}{\thead{\textbf{Performance \& Deployability}}}

\tabucline[1pt]{5-21}

& & & \multirow{2}{*}{\begin{turn}{90} \makecell[c]{\scriptsize Topology} \end{turn}} %{\begin{turn}{90} \makecell[c]{\scriptsize Direction} \end{turn}} \\
& \multicolumn{3}{c|}{\thead{\textbf{\makecell{Connection \\ Type}}}} 
& \multicolumn{2}{c|[1.5pt]}{\thead{\textbf{Symmetry}}}
& \multicolumn{2}{c|[1.5pt]}{\thead{\textbf{\makecell{Information \\ Description}}}}
& \multicolumn{2}{c|[1.5pt]}{\thead{\textbf{\makecell{Information \\ Distribution}}}}
& & & & & & & &


\\ \tabucline[1pt]{5-16}

& &
&  %\makecell[c]{\begin{turn}{90} \makecell[c]{Topology} \end{turn}}

& \makecell[c]{\begin{turn}{90} \makecell[c]{\scriptsize Direction} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{\scriptsize Timing} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{\scriptsize Lifetime} \end{turn}}

& \makecell[c]{\begin{turn}{90} \makecell[c]{\scriptsize P2P} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{\scriptsize Hierarchy} \end{turn}}

& \makecell[c]{\begin{turn}{90} \makecell[c]{Network \\ View} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Information \\ Content} \end{turn}}

& \makecell[c]{\begin{turn}{90} \makecell[c]{Directory \\ Service} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Information \\ Update } \end{turn}}


& \makecell[c]{\begin{turn}{90} \makecell[c]{\scriptsize Routing \\ Type} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{\scriptsize Node \\ Selection} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{\scriptsize Scheduling} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Latency} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Msg conn. based} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Implemented} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{Code available} \end{turn}}
& \makecell[c]{\begin{turn}{90} \makecell[c]{TCP/IP Layer} \end{turn}}

\\ \hline


\multicolumn{1}{|c|}{\multirow{6}{*}{\thead{\emph{\textbf{Mixnet-based}} \\ \emph{\textbf{protocols}}}}}

& \multicolumn{1}{l|}{Chaum's MixNet}
& \cite{Chaum:1981:mixnets}
& \fullyc,\partiallyc & \bi & & & \no & & \full & & \yes & & \source & \deterministic & & \high & & \no & \no & -

\\ \cline{2-21} 

\multicolumn{1}{|c|}{}
& \multicolumn{1}{l|}{Cypherpunk}
& \cite{Parekh:1996}
& \fullyc & \bi & & & \no & & \full && \yes && \source & \nondetuni &   &  \high & & \yes & ? & -

\\ \cline{2-21} 

\multicolumn{1}{|c|}{}
& \multicolumn{1}{l|}{Mixmaster}
& \cite{moller:2003:mixmaster}
& \fullyc & \uni & & & \no  & & \full && \yes && \source & \nondetuni  &    &  \high & & \yes & ? & email 

\\ \cline{2-21}

\multicolumn{1}{|c|}{}
& \multicolumn{1}{l|}{Babel}
& \cite{Babel:1996}
& \fullyc & \bi  & & & \no & & \full && \yes && \source & \nondetuni  &   &  \high && \yes & ? & -

\\ \cline{2-21}

\multicolumn{1}{|c|}{}
& \multicolumn{1}{l|}{Mixminion}
& \cite{Danezis:2003:mixminion}
& \fullyc & \bi  & & & \no & & \full && \yes && \source & \nondetuni  &  &   \high && \yes & ? & -

%\\ \hline

\\ \cline{2-21}

\multicolumn{1}{|c|}{}
& \multicolumn{1}{l|}{Web Mixes}
& \cite{Berthold:2000:JAP}
& \partiallyc & \bi  & & & \no & & \full && \yes && \source & \deterministic &  &   \low && \yes & ? & -

\\ \hline


% Anonymity \recipient \both 
% \boxtimes (fully) \Box (partial)
\multicolumn{1}{|c|}{\multirow{4}{*}{\thead{\emph{\textbf{DCNet-based}} \\ \emph{\textbf{protocols}}}}}
& \multicolumn{1}{l|}{{Chaum's DCNet}}
& \cite{Chaum:1988:DCNets}
& \fullyc & \uni  & & & \yes & & \full && \yes && \source & \deterministic &   &  \high & & \no & ? & Application

\\ \cline{2-21} 

\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Herbivore}
& \cite{Goel:2003:Herbivore}
& \mostlyc & \uni  & & & \yes & & \partially && \yes && \source & \deterministic  &   &   \high & & \yes & ? & IP

\\ \cline{2-21}

\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Dissent}
& \cite{Corrigan-Gibbs:2010:Dissent}
& \fullyc & \uni  & & & \yes & & \full && \yes && \source & \deterministic  &    &   \high & & \yes & ? & Application

\\ \cline{2-21}

\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Verdict}
& \cite{Corrigan-Gibbs:2013}
& \mostlyc & \uni  & & & \yes & & \partially && \yes && \source & \deterministic  &   &    \high & & \yes & ? & Application

\\ \hline


\multicolumn{1}{|c|}{\multirow{2}{*}{\thead{\emph{\textbf{Onion/Garlic}} \\ \emph{\textbf{routing}}}}}
& \multicolumn{1}{l|}{Tor}
& \cite{Dingledine:2004:Tor}
& \mostlyc & \bi  & & & \no & & \full && \yes && \source & \nondetnonuni  &   &   \low & & \yes & \yes & TCP

\\ \cline{2-21}

\multicolumn{1}{|l|}{\multirow{2}{*}{}}
& \multicolumn{1}{l|}{I2P}
& \cite{Web:2014:I2P}
& \mostlyc & \uni  & & & \yes & & \full  && \yes && \source & \nondetnonuni  &   &   \low & & \yes & ? & TCP,UDP

%\\ \cline{2-23}

\\ \cline{2-21}

\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Pisces}
& \cite{Mittal:2013:Pisces}
& \partiallyc & \bi  & & & \yes & & \full && \no && \source & \nondetuni &   &   \low & & \no & \no & TCP,UDP

\\ \hline

% producer & consumer
\multicolumn{1}{|c|}{\multirow{3}{*}{\thead{\emph{\textbf{DHT routing}}}}}
& \multicolumn{1}{l|}{Freenet/Darknet}
& \cite{Clarke:2010:FN}
& \partiallyc & \bi  & & & \yes & & \partially  && \no && \source & \deterministic  &   &  - & & \yes & ? & Content sharing

\\ \cline{2-21}

\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Freenet/Opennet}
& \cite{Clarke:2001:FN}
& \partiallyc & \bi & & & \yes & & \partially  && \no && \hop & \deterministic  &  & - & & \yes & \yes & Content sharing

\\ \cline{2-21}

%\\ \hline


%\iffalse
%initiator and responder anonymity
\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Gnunet}
& \cite{Bennett:2002:GN}
& \mostlyc & \bi & & & \yes & & \partially && \no && \hop & \deterministic  &  &   - & & \yes & \yes & Content sharing

\\ \hline

%\fi


\multicolumn{1}{|c|}{\multirow{2}{*}{\thead{\emph{\textbf{NG Internet}}}}}
& \multicolumn{1}{l|}{LAP}
& \cite{Hsiao:2011:LAP}
& & \bi & & & \no & & \full & & \no && \hop & \deterministic  & &    \low & & \no & \no & -

\\ \cline{2-21}

\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Dovetail}
& \cite{Sankey:2014:Dovetail}
& & \bi & & & \no & & \full  & & & & \hop & \deterministic  &  &  \low & & \no & \no & -

\\ \hline


\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Crowds}
& \cite{Reiter:1998:Crowds}
& \fullyc & \bi & & & \yes & & \full & &  \yes & & \hop & \nondetnonuni & & \low & & \no & \no & TCP (web browsing)

\\ \hline


\multicolumn{1}{|l|}{}
& \multicolumn{1}{l|}{Tarzan}
& \cite{Freedman:2002:Tarzan}
& \mostlyc & \bi & & & \yes & & \partially & & \no & & \source & \nondetnonuni  &  & \low & & \no & \no & UDP

\\ \hline


\end{tabu}

\begin{minipage}{\linewidth}

\source Source routing \\
\hop Hop-by-hop routing \\

\yes Yes \\
\no No \\
\canbeboth Can be both \\

\deterministic Deterministic \\
\nondetuni Non-deterministic and uniform \\
\nondetnonuni Non-deterministic and non-uniform \\

\uni Uni-directional \\
\bi Bi-directional \\

\fullyc Fully-connected \\
\mostlyc Mostly-connected \\
\partiallyc Partially-connected \\
% \notc Not-connected ({\color{red} REMOVE: It will not happen}) \\

%\sender Sender anonymity \\
%\recipient Recipient anonymity ({\color{red} REMOVE: It will not happen}) \\
%\both Both sender and recipient anonymity \\

$N$ Number of nodes in the network \\
$k$ Clique size, where number of cliques are $\lfloor N/k \rfloor$ \\
$v$ Variable, where $ 1 < v < N$ \\

\full Full \\
\partially Partial \\
\mini Minimal \\

\low Low \\
\high High \\

- Not applicable \\

\todo[inline]{\color{blue}{Move Nodes Contacted after Node Selection.}}

\end{minipage}

\end{table}

\end{landscape}

\end{flushleft}

==> sections/usage.tex <==
\subsection{Usage of Protocols}
\label{sec:usage}

In this section, we provide applications of routing protocols.

